Performance degradation of ImageNet trained models by simple image transformations

ImageNet trained PyTorch models are generally preferred as the off-the-shelf models for direct use or for initialisation in most computer vision tasks. In this paper, we simply test a representative set of these convolution and transformer based models under many simple image transformations like horizontal shifting, vertical shifting, scaling, rotation, presence of Gaussian noise, cutout, horizontal flip and vertical flip and report the performance drop caused by such transformations. We find that even simple transformations like rotating the image by 10{\deg} or zooming in by 20% can reduce the top-1 accuracy of models like ResNet152 by 1%+. The code is available at https://github.com/harshm121/imagenet-transformation-degradation.

==> tables_transformations/cutout.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{cutout size (5)} & alexnet   & 56.30                      & 78.93                      & -0.37                                     & -0.18                                     & -0.21                                     & -0.14                                     \\ \cline{2-8} 
                                     & vgg11     & 68.83                      & 88.52                      & -0.27                                     & -0.12                                     & -0.18                                     & -0.11                                     \\ \cline{2-8} 
                                     & resnet18  & 69.54                      & 88.99                      & -0.31                                     & -0.10                                     & -0.22                                     & -0.09                                     \\ \cline{2-8} 
                                     & vgg13     & 69.72                      & 89.19                      & -0.28                                     & -0.06                                     & -0.20                                     & -0.06                                     \\ \cline{2-8} 
                                     & vgg16     & 71.38                      & 90.28                      & -0.29                                     & -0.11                                     & -0.21                                     & -0.10                                     \\ \cline{2-8} 
                                     & vgg19     & 72.25                      & 90.81                      & -0.16                                     & -0.07                                     & -0.12                                     & -0.06                                     \\ \cline{2-8} 
                                     & resnet34  & 73.04                      & 91.35                      & -0.37                                     & -0.07                                     & -0.27                                     & -0.06                                     \\ \cline{2-8} 
                                     & resnet50  & 75.95                      & 92.79                      & -0.23                                     & -0.08                                     & -0.18                                     & -0.08                                     \\ \cline{2-8} 
                                     & resnet101 & 77.17                      & 93.51                      & -0.26                                     & -0.04                                     & -0.20                                     & -0.04                                     \\ \cline{2-8} 
                                     & resnet152 & 78.23                      & 93.95                      & -0.10                                     & -0.10                                     & -0.08                                     & -0.10                                     \\ \hline
\multirow{10}{*}{cutout size (10)}  & alexnet   & 55.92                      & 78.58                      & -1.04                                     & -0.61                                     & -0.59                                     & -0.49                                     \\ \cline{2-8} 
                                     & vgg11     & 68.64                      & 88.30                      & -0.54                                     & -0.36                                     & -0.37                                     & -0.32                                     \\ \cline{2-8} 
                                     & resnet18  & 69.16                      & 88.76                      & -0.85                                     & -0.35                                     & -0.59                                     & -0.31                                     \\ \cline{2-8} 
                                     & vgg13     & 69.54                      & 89.01                      & -0.54                                     & -0.26                                     & -0.38                                     & -0.23                                     \\ \cline{2-8} 
                                     & vgg16     & 71.10                      & 90.07                      & -0.69                                     & -0.34                                     & -0.49                                     & -0.31                                     \\ \cline{2-8} 
                                     & vgg19     & 71.89                      & 90.59                      & -0.65                                     & -0.31                                     & -0.47                                     & -0.28                                     \\ \cline{2-8} 
                                     & resnet34  & 72.80                      & 91.04                      & -0.70                                     & -0.42                                     & -0.51                                     & -0.38                                     \\ \cline{2-8} 
                                     & resnet50  & 75.66                      & 92.62                      & -0.62                                     & -0.26                                     & -0.47                                     & -0.24                                     \\ \cline{2-8} 
                                     & resnet101 & 76.97                      & 93.30                      & -0.51                                     & -0.26                                     & -0.40                                     & -0.25                                     \\ \cline{2-8} 
                                     & resnet152 & 77.97                      & 93.86                      & -0.43                                     & -0.20                                     & -0.34                                     & -0.19                                     \\ \hline
\multirow{10}{*}{cutout size (20)}  & alexnet   & 54.12                      & 77.33                      & -4.22                                     & -2.19                                     & -2.39                                     & -1.73                                     \\ \cline{2-8} 
                                     & vgg11     & 67.63                      & 87.70                      & -2.01                                     & -1.04                                     & -1.38                                     & -0.92                                     \\ \cline{2-8} 
                                     & resnet18  & 67.80                      & 87.98                      & -2.80                                     & -1.23                                     & -1.95                                     & -1.10                                     \\ \cline{2-8} 
                                     & vgg13     & 68.62                      & 88.34                      & -1.86                                     & -1.02                                     & -1.30                                     & -0.91                                     \\ \cline{2-8} 
                                     & vgg16     & 70.06                      & 89.38                      & -2.14                                     & -1.11                                     & -1.53                                     & -1.01                                     \\ \cline{2-8} 
                                     & vgg19     & 70.87                      & 89.96                      & -2.06                                     & -1.00                                     & -1.49                                     & -0.91                                     \\ \cline{2-8} 
                                     & resnet34  & 71.42                      & 90.31                      & -2.58                                     & -1.21                                     & -1.89                                     & -1.11                                     \\ \cline{2-8} 
                                     & resnet50  & 74.42                      & 91.90                      & -2.24                                     & -1.04                                     & -1.71                                     & -0.97                                     \\ \cline{2-8} 
                                     & resnet101 & 75.98                      & 92.77                      & -1.80                                     & -0.83                                     & -1.40                                     & -0.78                                     \\ \cline{2-8} 
                                     & resnet152 & 77.13                      & 93.41                      & -1.50                                     & -0.68                                     & -1.17                                     & -0.64                                     \\ \hline
\multirow{10}{*}{cutout size (30)}  & alexnet   & 51.78                      & 75.02                      & -8.36                                     & -5.12                                     & -4.73                                     & -4.05                                     \\ \cline{2-8} 
                                     & vgg11     & 65.69                      & 86.48                      & -4.81                                     & -2.42                                     & -3.32                                     & -2.14                                     \\ \cline{2-8} 
                                     & resnet18  & 65.74                      & 86.42                      & -5.75                                     & -2.98                                     & -4.01                                     & -2.65                                     \\ \cline{2-8} 
                                     & vgg13     & 67.19                      & 87.20                      & -3.91                                     & -2.29                                     & -2.73                                     & -2.04                                     \\ \cline{2-8} 
                                     & vgg16     & 68.30                      & 88.26                      & -4.59                                     & -2.35                                     & -3.28                                     & -2.12                                     \\ \cline{2-8} 
                                     & vgg19     & 69.02                      & 88.60                      & -4.62                                     & -2.50                                     & -3.35                                     & -2.27                                     \\ \cline{2-8} 
                                     & resnet34  & 69.38                      & 88.83                      & -5.35                                     & -2.83                                     & -3.92                                     & -2.59                                     \\ \cline{2-8} 
                                     & resnet50  & 72.85                      & 90.86                      & -4.31                                     & -2.16                                     & -3.28                                     & -2.01                                     \\ \cline{2-8} 
                                     & resnet101 & 74.37                      & 91.76                      & -3.87                                     & -1.91                                     & -3.00                                     & -1.79                                     \\ \cline{2-8} 
                                     & resnet152 & 75.54                      & 92.62                      & -3.53                                     & -1.52                                     & -2.77                                     & -1.43                                     \\ \hline
\end{tabular}
\label{tab:cutout_size1}
\caption{Drop in accuracy on ImageNet val set by cutting out a square of pixels of h = x\% of height and w = x\% of width of the image.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{cutout size (40)} & alexnet   & 47.84                      & 71.32                      & -15.33                                    & -9.80                                     & -8.66                                     & -7.75                                     \\ \cline{2-8} 
                                    & vgg11     & 62.96                      & 84.49                      & -8.77                                     & -4.67                                     & -6.05                                     & -4.14                                     \\ \cline{2-8} 
                                    & resnet18  & 62.85                      & 83.89                      & -9.89                                     & -5.82                                     & -6.90                                     & -5.18                                     \\ \cline{2-8} 
                                    & vgg13     & 64.34                      & 85.40                      & -7.98                                     & -4.31                                     & -5.58                                     & -3.85                                     \\ \cline{2-8} 
                                    & vgg16     & 65.39                      & 86.15                      & -8.66                                     & -4.68                                     & -6.20                                     & -4.23                                     \\ \cline{2-8} 
                                    & vgg19     & 66.25                      & 86.61                      & -8.46                                     & -4.69                                     & -6.12                                     & -4.27                                     \\ \cline{2-8} 
                                    & resnet34  & 66.51                      & 86.58                      & -9.27                                     & -5.29                                     & -6.80                                     & -4.83                                     \\ \cline{2-8} 
                                    & resnet50  & 70.28                      & 89.17                      & -7.68                                     & -3.98                                     & -5.85                                     & -3.69                                     \\ \cline{2-8} 
                                    & resnet101 & 72.11                      & 90.05                      & -6.81                                     & -3.73                                     & -5.27                                     & -3.49                                     \\ \cline{2-8} 
                                    & resnet152 & 73.41                      & 91.21                      & -6.25                                     & -3.01                                     & -4.90                                     & -2.83                                     \\ \hline
\multirow{10}{*}{cutout size (50)} & alexnet   & 42.94                      & 66.20                      & -24.01                                    & -16.28                                    & -13.57                                    & -12.87                                    \\ \cline{2-8} 
                                    & vgg11     & 59.29                      & 81.16                      & -14.09                                    & -8.42                                     & -9.72                                     & -7.46                                     \\ \cline{2-8} 
                                    & resnet18  & 58.29                      & 80.14                      & -16.43                                    & -10.03                                    & -11.46                                    & -8.93                                     \\ \cline{2-8} 
                                    & vgg13     & 60.52                      & 82.19                      & -13.44                                    & -7.90                                     & -9.39                                     & -7.05                                     \\ \cline{2-8} 
                                    & vgg16     & 61.62                      & 82.83                      & -13.92                                    & -8.36                                     & -9.97                                     & -7.56                                     \\ \cline{2-8} 
                                    & vgg19     & 61.87                      & 83.06                      & -14.50                                    & -8.60                                     & -10.49                                    & -7.81                                     \\ \cline{2-8} 
                                    & resnet34  & 62.24                      & 83.08                      & -15.10                                    & -9.12                                     & -11.07                                    & -8.34                                     \\ \cline{2-8} 
                                    & resnet50  & 66.43                      & 86.30                      & -12.74                                    & -7.07                                     & -9.70                                     & -6.57                                     \\ \cline{2-8} 
                                    & resnet101 & 68.55                      & 87.58                      & -11.40                                    & -6.38                                     & -8.82                                     & -5.97                                     \\ \cline{2-8} 
                                    & resnet152 & 69.98                      & 88.39                      & -10.63                                    & -6.01                                     & -8.32                                     & -5.66                                     \\ \hline
\end{tabular}
\label{tab:cutout_size2}
\caption{Drop in accuracy on ImageNet val set by cutting out a square of pixels of h = x\% of height and w = x\% of width of the image.}
\end{table*}

==> tables_transformations/cutout_num.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{cutout num 1} & alexnet   & 54.11                      & 77.36                      & -4.24                                     & -2.16                                     & -2.40                                     & -1.71                                     \\ \cline{2-8} 
                               & vgg11     & 67.49                      & 87.72                      & -2.21                                     & -1.03                                     & -1.52                                     & -0.91                                     \\ \cline{2-8} 
                               & resnet18  & 68.08                      & 87.78                      & -2.40                                     & -1.45                                     & -1.67                                     & -1.29                                     \\ \cline{2-8} 
                               & vgg13     & 68.51                      & 88.37                      & -2.01                                     & -0.98                                     & -1.41                                     & -0.88                                     \\ \cline{2-8} 
                               & vgg16     & 70.17                      & 89.46                      & -1.98                                     & -1.02                                     & -1.42                                     & -0.92                                     \\ \cline{2-8} 
                               & vgg19     & 70.95                      & 89.88                      & -1.95                                     & -1.09                                     & -1.41                                     & -0.99                                     \\ \cline{2-8} 
                               & resnet34  & 71.36                      & 90.05                      & -2.65                                     & -1.50                                     & -1.95                                     & -1.37                                     \\ \cline{2-8} 
                               & resnet50  & 74.58                      & 92.01                      & -2.03                                     & -0.92                                     & -1.54                                     & -0.86                                     \\ \cline{2-8} 
                               & resnet101 & 75.77                      & 92.75                      & -2.07                                     & -0.85                                     & -1.60                                     & -0.80                                     \\ \cline{2-8} 
                               & resnet152 & 77.16                      & 93.43                      & -1.47                                     & -0.66                                     & -1.15                                     & -0.62                                     \\ \hline
\multirow{10}{*}{cutout num 2} & alexnet   & 51.41                      & 74.77                      & -9.01                                     & -5.43                                     & -5.09                                     & -4.30                                     \\ \cline{2-8} 
                               & vgg11     & 65.57                      & 86.48                      & -4.99                                     & -2.42                                     & -3.44                                     & -2.14                                     \\ \cline{2-8} 
                               & resnet18  & 65.57                      & 86.29                      & -6.00                                     & -3.12                                     & -4.18                                     & -2.78                                     \\ \cline{2-8} 
                               & vgg13     & 66.77                      & 87.11                      & -4.51                                     & -2.39                                     & -3.15                                     & -2.13                                     \\ \cline{2-8} 
                               & vgg16     & 68.05                      & 88.11                      & -4.94                                     & -2.52                                     & -3.53                                     & -2.28                                     \\ \cline{2-8} 
                               & vgg19     & 68.89                      & 88.47                      & -4.80                                     & -2.64                                     & -3.47                                     & -2.40                                     \\ \cline{2-8} 
                               & resnet34  & 69.02                      & 88.56                      & -5.85                                     & -3.13                                     & -4.29                                     & -2.86                                     \\ \cline{2-8} 
                               & resnet50  & 72.76                      & 90.84                      & -4.42                                     & -2.18                                     & -3.37                                     & -2.02                                     \\ \cline{2-8} 
                               & resnet101 & 74.36                      & 91.70                      & -3.89                                     & -1.98                                     & -3.01                                     & -1.85                                     \\ \cline{2-8} 
                               & resnet152 & 75.75                      & 92.56                      & -3.27                                     & -1.58                                     & -2.56                                     & -1.48                                     \\ \hline
\multirow{10}{*}{cutout num 3} & alexnet   & 48.01                      & 72.03                      & -15.04                                    & -8.89                                     & -8.50                                     & -7.03                                     \\ \cline{2-8} 
                               & vgg11     & 63.51                      & 85.04                      & -7.98                                     & -4.05                                     & -5.51                                     & -3.59                                     \\ \cline{2-8} 
                               & resnet18  & 63.20                      & 84.41                      & -9.39                                     & -5.23                                     & -6.55                                     & -4.66                                     \\ \cline{2-8} 
                               & vgg13     & 64.74                      & 85.73                      & -7.41                                     & -3.93                                     & -5.18                                     & -3.51                                     \\ \cline{2-8} 
                               & vgg16     & 65.67                      & 86.50                      & -8.26                                     & -4.30                                     & -5.91                                     & -3.89                                     \\ \cline{2-8} 
                               & vgg19     & 66.53                      & 86.90                      & -8.06                                     & -4.38                                     & -5.83                                     & -3.98                                     \\ \cline{2-8} 
                               & resnet34  & 66.50                      & 86.68                      & -9.29                                     & -5.18                                     & -6.81                                     & -4.74                                     \\ \cline{2-8} 
                               & resnet50  & 70.29                      & 89.35                      & -7.67                                     & -3.78                                     & -5.84                                     & -3.51                                     \\ \cline{2-8} 
                               & resnet101 & 72.23                      & 90.47                      & -6.65                                     & -3.29                                     & -5.14                                     & -3.07                                     \\ \cline{2-8} 
                               & resnet152 & 74.15                      & 91.62                      & -5.31                                     & -2.58                                     & -4.16                                     & -2.42                                     \\ \hline
\multirow{10}{*}{cutout num 4} & alexnet   & 44.50                      & 68.40                      & -21.25                                    & -13.50                                    & -12.01                                    & -10.67                                    \\ \cline{2-8} 
                               & vgg11     & 60.94                      & 82.97                      & -11.70                                    & -6.38                                     & -8.08                                     & -5.65                                     \\ \cline{2-8} 
                               & resnet18  & 60.36                      & 82.25                      & -13.47                                    & -7.66                                     & -9.40                                     & -6.82                                     \\ \cline{2-8} 
                               & vgg13     & 62.34                      & 83.66                      & -10.84                                    & -6.26                                     & -7.58                                     & -5.58                                     \\ \cline{2-8} 
                               & vgg16     & 63.23                      & 84.56                      & -11.67                                    & -6.44                                     & -8.35                                     & -5.82                                     \\ \cline{2-8} 
                               & vgg19     & 64.09                      & 85.02                      & -11.44                                    & -6.44                                     & -8.28                                     & -5.85                                     \\ \cline{2-8} 
                               & resnet34  & 63.64                      & 84.51                      & -13.19                                    & -7.55                                     & -9.67                                     & -6.91                                     \\ \cline{2-8} 
                               & resnet50  & 68.22                      & 87.77                      & -10.38                                    & -5.49                                     & -7.90                                     & -5.09                                     \\ \cline{2-8} 
                               & resnet101 & 70.59                      & 89.15                      & -8.77                                     & -4.70                                     & -6.78                                     & -4.39                                     \\ \cline{2-8} 
                               & resnet152 & 72.53                      & 90.61                      & -7.38                                     & -3.66                                     & -5.78                                     & -3.44                                     \\ \hline
\end{tabular}
\label{tab:cutout_num}
\caption{Drop in accuracy on ImageNet val set by cutting out a x number of squares of pixels of h = 20\% of height and w = 20\% of width of the image.}
\end{table*}

==> tables_transformations/noise.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{gaussian noise (variance = 0.05*255)} & alexnet   & 53.63                      & 76.75                      & -5.10                                     & -2.93                                     & -2.88                                     & -2.32                                     \\ \cline{2-8} 
                                                       & vgg11     & 65.03                      & 86.15                      & -5.78                                     & -2.80                                     & -3.99                                     & -2.48                                     \\ \cline{2-8} 
                                                       & resnet18  & 66.64                      & 87.08                      & -4.46                                     & -2.24                                     & -3.11                                     & -1.99                                     \\ \cline{2-8} 
                                                       & vgg13     & 65.80                      & 86.66                      & -5.89                                     & -2.89                                     & -4.12                                     & -2.58                                     \\ \cline{2-8} 
                                                       & vgg16     & 68.00                      & 88.09                      & -5.01                                     & -2.54                                     & -3.59                                     & -2.29                                     \\ \cline{2-8} 
                                                       & vgg19     & 68.65                      & 88.61                      & -5.14                                     & -2.50                                     & -3.72                                     & -2.27                                     \\ \cline{2-8} 
                                                       & resnet34  & 70.64                      & 90.00                      & -3.64                                     & -1.55                                     & -2.67                                     & -1.42                                     \\ \cline{2-8} 
                                                       & resnet50  & 73.20                      & 91.34                      & -3.84                                     & -1.64                                     & -2.93                                     & -1.52                                     \\ \cline{2-8} 
                                                       & resnet101 & 75.29                      & 92.50                      & -2.69                                     & -1.12                                     & -2.08                                     & -1.05                                     \\ \cline{2-8} 
                                                       & resnet152 & 76.25                      & 93.05                      & -2.62                                     & -1.05                                     & -2.05                                     & -0.99                                     \\ \hline
\multirow{10}{*}{gaussian noise (variance = 0.1*255)}  & alexnet   & 44.62                      & 68.45                      & -21.04                                    & -13.43                                    & -11.89                                    & -10.62                                    \\ \cline{2-8} 
                                                       & vgg11     & 56.47                      & 79.71                      & -18.17                                    & -10.06                                    & -12.54                                    & -8.92                                     \\ \cline{2-8} 
                                                       & resnet18  & 59.92                      & 82.21                      & -14.10                                    & -7.70                                     & -9.84                                     & -6.86                                     \\ \cline{2-8} 
                                                       & vgg13     & 56.74                      & 79.70                      & -18.85                                    & -10.70                                    & -13.18                                    & -9.55                                     \\ \cline{2-8} 
                                                       & vgg16     & 60.26                      & 82.65                      & -15.82                                    & -8.55                                     & -11.33                                    & -7.73                                     \\ \cline{2-8} 
                                                       & vgg19     & 61.17                      & 83.10                      & -15.47                                    & -8.55                                     & -11.20                                    & -7.77                                     \\ \cline{2-8} 
                                                       & resnet34  & 65.93                      & 86.68                      & -10.06                                    & -5.18                                     & -7.37                                     & -4.74                                     \\ \cline{2-8} 
                                                       & resnet50  & 68.23                      & 87.99                      & -10.37                                    & -5.25                                     & -7.90                                     & -4.87                                     \\ \cline{2-8} 
                                                       & resnet101 & 70.79                      & 89.95                      & -8.51                                     & -3.85                                     & -6.58                                     & -3.60                                     \\ \cline{2-8} 
                                                       & resnet152 & 72.33                      & 90.87                      & -7.64                                     & -3.38                                     & -5.98                                     & -3.18                                     \\ \hline
\multirow{10}{*}{gaussian noise (variance = 0.2*255)}  & alexnet   & 22.99                      & 42.46                      & -59.32                                    & -46.30                                    & -33.52                                    & -36.61                                    \\ \cline{2-8} 
                                                       & vgg11     & 33.51                      & 57.30                      & -51.44                                    & -35.35                                    & -35.50                                    & -31.33                                    \\ \cline{2-8} 
                                                       & resnet18  & 42.01                      & 66.12                      & -39.77                                    & -25.77                                    & -27.74                                    & -22.96                                    \\ \cline{2-8} 
                                                       & vgg13     & 31.01                      & 53.70                      & -55.65                                    & -39.82                                    & -38.91                                    & -35.54                                    \\ \cline{2-8} 
                                                       & vgg16     & 37.69                      & 61.83                      & -47.35                                    & -31.59                                    & -33.90                                    & -28.56                                    \\ \cline{2-8} 
                                                       & vgg19     & 39.85                      & 63.75                      & -44.93                                    & -29.85                                    & -32.51                                    & -27.12                                    \\ \cline{2-8} 
                                                       & resnet34  & 51.68                      & 75.03                      & -29.51                                    & -17.93                                    & -21.63                                    & -16.39                                    \\ \cline{2-8} 
                                                       & resnet50  & 52.95                      & 76.31                      & -30.45                                    & -17.82                                    & -23.18                                    & -16.55                                    \\ \cline{2-8} 
                                                       & resnet101 & 58.23                      & 80.68                      & -24.74                                    & -13.75                                    & -19.14                                    & -12.86                                    \\ \cline{2-8} 
                                                       & resnet152 & 61.60                      & 83.44                      & -21.34                                    & -11.28                                    & -16.71                                    & -10.60                                    \\ \hline
\multirow{10}{*}{gaussian noise (variance = 0.3*255)}  & alexnet   & 9.28                       & 20.43                      & -83.58                                    & -74.16                                    & -47.23                                    & -58.63                                    \\ \cline{2-8} 
                                                       & vgg11     & 15.18                      & 31.70                      & -78.00                                    & -64.23                                    & -53.83                                    & -56.92                                    \\ \cline{2-8} 
                                                       & resnet18  & 24.16                      & 45.24                      & -65.37                                    & -49.21                                    & -45.60                                    & -43.83                                    \\ \cline{2-8} 
                                                       & vgg13     & 12.48                      & 26.10                      & -82.15                                    & -70.76                                    & -57.44                                    & -63.15                                    \\ \cline{2-8} 
                                                       & vgg16     & 18.27                      & 36.59                      & -74.47                                    & -59.52                                    & -53.31                                    & -53.80                                    \\ \cline{2-8} 
                                                       & vgg19     & 19.94                      & 38.84                      & -72.45                                    & -57.26                                    & -52.43                                    & -52.03                                    \\ \cline{2-8} 
                                                       & resnet34  & 33.05                      & 55.75                      & -54.91                                    & -39.01                                    & -40.26                                    & -35.67                                    \\ \cline{2-8} 
                                                       & resnet50  & 35.56                      & 58.88                      & -53.28                                    & -36.59                                    & -40.56                                    & -33.98                                    \\ \cline{2-8} 
                                                       & resnet101 & 42.83                      & 66.46                      & -44.65                                    & -28.96                                    & -34.55                                    & -27.09                                    \\ \cline{2-8} 
                                                       & resnet152 & 47.25                      & 70.62                      & -39.67                                    & -24.90                                    & -31.06                                    & -23.42                                    \\ \hline
\end{tabular}
\label{tab:noise}
\caption{Drop in accuracy on ImageNet val set by adding guassian noise of varying variance to pixel values}
\end{table*}


\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{gaussian noise (variance = 0.05*255)} & alexnet   & 53.63                      & 76.75                      & -5.10                                     & -2.93                                     & -2.88                                     & -2.32                                     \\ \cline{2-8} 
                                                       & vgg11     & 65.03                      & 86.15                      & -5.78                                     & -2.80                                     & -3.99                                     & -2.48                                     \\ \cline{2-8} 
                                                       & resnet18  & 66.64                      & 87.08                      & -4.46                                     & -2.24                                     & -3.11                                     & -1.99                                     \\ \cline{2-8} 
                                                       & vgg13     & 65.80                      & 86.66                      & -5.89                                     & -2.89                                     & -4.12                                     & -2.58                                     \\ \cline{2-8} 
                                                       & vgg16     & 68.00                      & 88.09                      & -5.01                                     & -2.54                                     & -3.59                                     & -2.29                                     \\ \cline{2-8} 
                                                       & vgg19     & 68.65                      & 88.61                      & -5.14                                     & -2.50                                     & -3.72                                     & -2.27                                     \\ \cline{2-8} 
                                                       & resnet34  & 70.64                      & 90.00                      & -3.64                                     & -1.55                                     & -2.67                                     & -1.42                                     \\ \cline{2-8} 
                                                       & resnet50  & 73.20                      & 91.34                      & -3.84                                     & -1.64                                     & -2.93                                     & -1.52                                     \\ \cline{2-8} 
                                                       & resnet101 & 75.29                      & 92.50                      & -2.69                                     & -1.12                                     & -2.08                                     & -1.05                                     \\ \cline{2-8} 
                                                       & resnet152 & 76.25                      & 93.05                      & -2.62                                     & -1.05                                     & -2.05                                     & -0.99                                     \\ \hline
\multirow{10}{*}{gaussian noise (variance = 0.1*255)}  & alexnet   & 44.62                      & 68.45                      & -21.04                                    & -13.43                                    & -11.89                                    & -10.62                                    \\ \cline{2-8} 
                                                       & vgg11     & 56.47                      & 79.71                      & -18.17                                    & -10.06                                    & -12.54                                    & -8.92                                     \\ \cline{2-8} 
                                                       & resnet18  & 59.92                      & 82.21                      & -14.10                                    & -7.70                                     & -9.84                                     & -6.86                                     \\ \cline{2-8} 
                                                       & vgg13     & 56.74                      & 79.70                      & -18.85                                    & -10.70                                    & -13.18                                    & -9.55                                     \\ \cline{2-8} 
                                                       & vgg16     & 60.26                      & 82.65                      & -15.82                                    & -8.55                                     & -11.33                                    & -7.73                                     \\ \cline{2-8} 
                                                       & vgg19     & 61.17                      & 83.10                      & -15.47                                    & -8.55                                     & -11.20                                    & -7.77                                     \\ \cline{2-8} 
                                                       & resnet34  & 65.93                      & 86.68                      & -10.06                                    & -5.18                                     & -7.37                                     & -4.74                                     \\ \cline{2-8} 
                                                       & resnet50  & 68.23                      & 87.99                      & -10.37                                    & -5.25                                     & -7.90                                     & -4.87                                     \\ \cline{2-8} 
                                                       & resnet101 & 70.79                      & 89.95                      & -8.51                                     & -3.85                                     & -6.58                                     & -3.60                                     \\ \cline{2-8} 
                                                       & resnet152 & 72.33                      & 90.87                      & -7.64                                     & -3.38                                     & -5.98                                     & -3.18                                     \\ \hline
\multirow{10}{*}{gaussian noise (variance = 0.2*255)}  & alexnet   & 22.99                      & 42.46                      & -59.32                                    & -46.30                                    & -33.52                                    & -36.61                                    \\ \cline{2-8} 
                                                       & vgg11     & 33.51                      & 57.30                      & -51.44                                    & -35.35                                    & -35.50                                    & -31.33                                    \\ \cline{2-8} 
                                                       & resnet18  & 42.01                      & 66.12                      & -39.77                                    & -25.77                                    & -27.74                                    & -22.96                                    \\ \cline{2-8} 
                                                       & vgg13     & 31.01                      & 53.70                      & -55.65                                    & -39.82                                    & -38.91                                    & -35.54                                    \\ \cline{2-8} 
                                                       & vgg16     & 37.69                      & 61.83                      & -47.35                                    & -31.59                                    & -33.90                                    & -28.56                                    \\ \cline{2-8} 
                                                       & vgg19     & 39.85                      & 63.75                      & -44.93                                    & -29.85                                    & -32.51                                    & -27.12                                    \\ \cline{2-8} 
                                                       & resnet34  & 51.68                      & 75.03                      & -29.51                                    & -17.93                                    & -21.63                                    & -16.39                                    \\ \cline{2-8} 
                                                       & resnet50  & 52.95                      & 76.31                      & -30.45                                    & -17.82                                    & -23.18                                    & -16.55                                    \\ \cline{2-8} 
                                                       & resnet101 & 58.23                      & 80.68                      & -24.74                                    & -13.75                                    & -19.14                                    & -12.86                                    \\ \cline{2-8} 
                                                       & resnet152 & 61.60                      & 83.44                      & -21.34                                    & -11.28                                    & -16.71                                    & -10.60                                    \\ \hline
\multirow{10}{*}{gaussian noise (variance = 0.3*255)}  & alexnet   & 9.28                       & 20.43                      & -83.58                                    & -74.16                                    & -47.23                                    & -58.63                                    \\ \cline{2-8} 
                                                       & vgg11     & 15.18                      & 31.70                      & -78.00                                    & -64.23                                    & -53.83                                    & -56.92                                    \\ \cline{2-8} 
                                                       & resnet18  & 24.16                      & 45.24                      & -65.37                                    & -49.21                                    & -45.60                                    & -43.83                                    \\ \cline{2-8} 
                                                       & vgg13     & 12.48                      & 26.10                      & -82.15                                    & -70.76                                    & -57.44                                    & -63.15                                    \\ \cline{2-8} 
                                                       & vgg16     & 18.27                      & 36.59                      & -74.47                                    & -59.52                                    & -53.31                                    & -53.80                                    \\ \cline{2-8} 
                                                       & vgg19     & 19.94                      & 38.84                      & -72.45                                    & -57.26                                    & -52.43                                    & -52.03                                    \\ \cline{2-8} 
                                                       & resnet34  & 33.05                      & 55.75                      & -54.91                                    & -39.01                                    & -40.26                                    & -35.67                                    \\ \cline{2-8} 
                                                       & resnet50  & 35.56                      & 58.88                      & -53.28                                    & -36.59                                    & -40.56                                    & -33.98                                    \\ \cline{2-8} 
                                                       & resnet101 & 42.83                      & 66.46                      & -44.65                                    & -28.96                                    & -34.55                                    & -27.09                                    \\ \cline{2-8} 
                                                       & resnet152 & 47.25                      & 70.62                      & -39.67                                    & -24.90                                    & -31.06                                    & -23.42                                    \\ \hline
\end{tabular}
\label{tab:gaussian_noise}
\caption{Drop in accuracy on ImageNet val set by adding random guassian noise to each pixel}
\end{table*}

==> tables_transformations/original.tex <==
\begin{table*}[h]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Models    & Top 1 accuracy & Top 1 reported accuracy & \% difference & Top 5 accuracy & Top 5 reported accuracy &\% difference \\ \hline
alexnet   & 56.506         & 56.522                                                             & 0.028\%           & 79.066 & 79.066                                                             & 0.000\%           \\ \hline
vgg11     & 69.012         & 69.02                                                              & 0.012\%           & 88.626 & 88.628                                                             & 0.002\%           \\ \hline
resnet18  & 69.752         & 69.758                                                             & 0.009\%           & 89.074 & 89.078                                                             & 0.004\%           \\ \hline
vgg13     & 69.918         & 69.928                                                             & 0.014\%           & 89.244 & 89.246                                                             & 0.002\%           \\ \hline
vgg16     & 71.588         & 71.592                                                             & 0.006\%           & 90.382 & 90.382                                                             & 0.000\%           \\ \hline
vgg19     & 72.366         & 72.376                                                             & 0.014\%           & 90.874 & 90.876                                                             & 0.002\%           \\ \hline
resnet34  & 73.308         & 73.314                                                             & 0.008\%           & 91.418 & 91.42                                                              & 0.002\%           \\ \hline
resnet50  & 76.128         & 76.13                                                              & 0.003\%           & 92.862 & 92.862                                                             & 0.000\%           \\ \hline
resnet101 & 77.372         & 77.374                                                             & 0.003\%           & 93.546 & 93.546                                                             & 0.000\%           \\ \hline
resnet152 & 78.308         & 78.312                                                             & 0.005\%           & 94.046 & 94.046                                                             & 0.000\%           \\ \hline
\end{tabular}
\caption{The top-1 and top-5 accuracies evaluated as compared to the ones reported on the PyTorch vision website \cite{pytorch}.}
\label{tab:reproduce}
\end{table*}

==> tables_transformations/rotate.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
Transformation               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{rotate +10}  & alexnet   & 53.78                      & 76.89                      & -4.83                                     & -2.75                                     & -2.73                                     & -2.17                                     \\ \cline{2-8} 
                              & vgg11     & 66.89                      & 87.36                      & -3.08                                     & -1.43                                     & -2.12                                     & -1.27                                     \\ \cline{2-8} 
                              & resnet18  & 67.83                      & 87.86                      & -2.75                                     & -1.37                                     & -1.92                                     & -1.22                                     \\ \cline{2-8} 
                              & vgg13     & 67.64                      & 87.92                      & -3.26                                     & -1.48                                     & -2.28                                     & -1.32                                     \\ \cline{2-8} 
                              & vgg16     & 69.67                      & 89.25                      & -2.68                                     & -1.25                                     & -1.92                                     & -1.13                                     \\ \cline{2-8} 
                              & vgg19     & 70.56                      & 89.74                      & -2.50                                     & -1.25                                     & -1.81                                     & -1.13                                     \\ \cline{2-8} 
                              & resnet34  & 71.66                      & 90.24                      & -2.24                                     & -1.29                                     & -1.64                                     & -1.18                                     \\ \cline{2-8} 
                              & resnet50  & 74.52                      & 91.96                      & -2.11                                     & -0.97                                     & -1.61                                     & -0.90                                     \\ \cline{2-8} 
                              & resnet101 & 76.02                      & 92.79                      & -1.75                                     & -0.80                                     & -1.36                                     & -0.75                                     \\ \cline{2-8} 
                              & resnet152 & 77.08                      & 93.37                      & -1.57                                     & -0.71                                     & -1.23                                     & -0.67                                     \\ \hline
\multirow{10}{*}{rotate +25} & alexnet   & 42.16                      & 65.69                      & -25.38                                    & -16.92                                    & -14.34                                    & -13.38                                    \\ \cline{2-8} 
                              & vgg11     & 58.63                      & 81.19                      & -15.04                                    & -8.39                                     & -10.38                                    & -7.44                                     \\ \cline{2-8} 
                              & resnet18  & 60.97                      & 82.93                      & -12.60                                    & -6.89                                     & -8.79                                     & -6.14                                     \\ \cline{2-8} 
                              & vgg13     & 60.21                      & 82.31                      & -13.88                                    & -7.77                                     & -9.70                                     & -6.94                                     \\ \cline{2-8} 
                              & vgg16     & 62.91                      & 84.24                      & -12.13                                    & -6.80                                     & -8.68                                     & -6.14                                     \\ \cline{2-8} 
                              & vgg19     & 63.74                      & 84.91                      & -11.92                                    & -6.56                                     & -8.63                                     & -5.96                                     \\ \cline{2-8} 
                              & resnet34  & 65.20                      & 85.63                      & -11.06                                    & -6.33                                     & -8.11                                     & -5.79                                     \\ \cline{2-8} 
                              & resnet50  & 69.40                      & 88.54                      & -8.84                                     & -4.66                                     & -6.73                                     & -4.32                                     \\ \cline{2-8} 
                              & resnet101 & 71.38                      & 89.83                      & -7.74                                     & -3.98                                     & -5.99                                     & -3.72                                     \\ \cline{2-8} 
                              & resnet152 & 73.24                      & 91.27                      & -6.48                                     & -2.95                                     & -5.07                                     & -2.77                                     \\ \hline
\multirow{10}{*}{rotate +45}  & alexnet   & 31.67                      & 53.00                      & -43.96                                    & -32.97                                    & -24.84                                    & -26.07                                    \\ \cline{2-8} 
                              & vgg11     & 48.52                      & 71.90                      & -29.70                                    & -18.88                                    & -20.49                                    & -16.73                                    \\ \cline{2-8} 
                              & resnet18  & 50.70                      & 74.08                      & -27.31                                    & -16.83                                    & -19.05                                    & -14.99                                    \\ \cline{2-8} 
                              & vgg13     & 50.47                      & 74.27                      & -27.81                                    & -16.78                                    & -19.45                                    & -14.98                                    \\ \cline{2-8} 
                              & vgg16     & 52.86                      & 76.04                      & -26.16                                    & -15.87                                    & -18.72                                    & -14.34                                    \\ \cline{2-8} 
                              & vgg19     & 53.05                      & 76.19                      & -26.69                                    & -16.16                                    & -19.32                                    & -14.69                                    \\ \cline{2-8} 
                              & resnet34  & 54.74                      & 77.22                      & -25.33                                    & -15.53                                    & -18.57                                    & -14.20                                    \\ \cline{2-8} 
                              & resnet50  & 60.85                      & 82.31                      & -20.07                                    & -11.36                                    & -15.28                                    & -10.55                                    \\ \cline{2-8} 
                              & resnet101 & 63.31                      & 84.25                      & -18.17                                    & -9.94                                     & -14.06                                    & -9.30                                     \\ \cline{2-8} 
                              & resnet152 & 65.90                      & 86.41                      & -15.85                                    & -8.12                                     & -12.41                                    & -7.64                                     \\ \hline
\multirow{10}{*}{rotate +90}  & alexnet   & 27.20                      & 48.71                      & -51.86                                    & -38.39                                    & -29.30                                    & -30.35                                    \\ \cline{2-8} 
                              & vgg11     & 40.13                      & 64.01                      & -41.85                                    & -27.78                                    & -28.88                                    & -24.62                                    \\ \cline{2-8} 
                              & resnet18  & 40.21                      & 63.84                      & -42.35                                    & -28.33                                    & -29.54                                    & -25.24                                    \\ \cline{2-8} 
                              & vgg13     & 41.61                      & 65.62                      & -40.49                                    & -26.47                                    & -28.31                                    & -23.63                                    \\ \cline{2-8} 
                              & vgg16     & 42.82                      & 66.63                      & -40.19                                    & -26.28                                    & -28.77                                    & -23.75                                    \\ \cline{2-8} 
                              & vgg19     & 42.89                      & 67.04                      & -40.73                                    & -26.23                                    & -29.47                                    & -23.84                                    \\ \cline{2-8} 
                              & resnet34  & 43.57                      & 67.31                      & -40.57                                    & -26.37                                    & -29.74                                    & -24.11                                    \\ \cline{2-8} 
                              & resnet50  & 49.71                      & 73.06                      & -34.71                                    & -21.32                                    & -26.42                                    & -19.80                                    \\ \cline{2-8} 
                              & resnet101 & 51.48                      & 74.47                      & -33.47                                    & -20.39                                    & -25.90                                    & -19.07                                    \\ \cline{2-8} 
                              & resnet152 & 53.39                      & 75.95                      & -31.82                                    & -19.24                                    & -24.92                                    & -18.10                                    \\ \hline
\end{tabular}
\label{tab:rotate_pos}
\caption{Drop in accuracy on ImageNet val set by rotating the images (degrees in clockwise direction)}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
Transformation               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{rotate -10} & alexnet   & 53.59                      & 76.81                      & -5.16                                     & -2.85                                     & -2.92                                     & -2.25                                     \\ \cline{2-8} 
                             & vgg11     & 66.80                      & 87.31                      & -3.21                                     & -1.48                                     & -2.21                                     & -1.32                                     \\ \cline{2-8} 
                             & resnet18  & 67.84                      & 87.93                      & -2.75                                     & -1.29                                     & -1.92                                     & -1.15                                     \\ \cline{2-8} 
                             & vgg13     & 67.86                      & 87.89                      & -2.95                                     & -1.52                                     & -2.06                                     & -1.36                                     \\ \cline{2-8} 
                             & vgg16     & 69.89                      & 89.31                      & -2.37                                     & -1.18                                     & -1.70                                     & -1.07                                     \\ \cline{2-8} 
                             & vgg19     & 70.54                      & 89.71                      & -2.53                                     & -1.29                                     & -1.83                                     & -1.17                                     \\ \cline{2-8} 
                             & resnet34  & 71.48                      & 90.36                      & -2.49                                     & -1.16                                     & -1.83                                     & -1.06                                     \\ \cline{2-8} 
                             & resnet50  & 74.48                      & 91.85                      & -2.16                                     & -1.09                                     & -1.65                                     & -1.01                                     \\ \cline{2-8} 
                             & resnet101 & 75.88                      & 92.80                      & -1.93                                     & -0.80                                     & -1.49                                     & -0.75                                     \\ \cline{2-8} 
                             & resnet152 & 76.93                      & 93.38                      & -1.76                                     & -0.71                                     & -1.38                                     & -0.66                                     \\ \hline
\multirow{10}{*}{rotate -25} & alexnet   & 42.07                      & 65.32                      & -25.54                                    & -17.39                                    & -14.43                                    & -13.75                                    \\ \cline{2-8} 
                             & vgg11     & 58.77                      & 81.30                      & -14.84                                    & -8.27                                     & -10.24                                    & -7.33                                     \\ \cline{2-8} 
                             & resnet18  & 61.02                      & 82.83                      & -12.52                                    & -7.01                                     & -8.73                                     & -6.24                                     \\ \cline{2-8} 
                             & vgg13     & 60.55                      & 82.69                      & -13.40                                    & -7.35                                     & -9.37                                     & -6.56                                     \\ \cline{2-8} 
                             & vgg16     & 62.90                      & 84.33                      & -12.13                                    & -6.69                                     & -8.69                                     & -6.05                                     \\ \cline{2-8} 
                             & vgg19     & 63.59                      & 84.97                      & -12.13                                    & -6.50                                     & -8.78                                     & -5.91                                     \\ \cline{2-8} 
                             & resnet34  & 65.06                      & 85.70                      & -11.26                                    & -6.25                                     & -8.25                                     & -5.71                                     \\ \cline{2-8} 
                             & resnet50  & 69.47                      & 88.63                      & -8.75                                     & -4.56                                     & -6.66                                     & -4.23                                     \\ \cline{2-8} 
                             & resnet101 & 71.41                      & 89.98                      & -7.71                                     & -3.81                                     & -5.96                                     & -3.56                                     \\ \cline{2-8} 
                             & resnet152 & 73.13                      & 91.15                      & -6.61                                     & -3.08                                     & -5.17                                     & -2.90                                     \\ \hline
\multirow{10}{*}{rotate -45} & alexnet   & 31.65                      & 53.06                      & -43.99                                    & -32.89                                    & -24.86                                    & -26.00                                    \\ \cline{2-8} 
                             & vgg11     & 48.30                      & 71.99                      & -30.01                                    & -18.77                                    & -20.71                                    & -16.64                                    \\ \cline{2-8} 
                             & resnet18  & 50.71                      & 74.13                      & -27.30                                    & -16.77                                    & -19.04                                    & -14.94                                    \\ \cline{2-8} 
                             & vgg13     & 50.55                      & 74.18                      & -27.71                                    & -16.88                                    & -19.37                                    & -15.07                                    \\ \cline{2-8} 
                             & vgg16     & 52.78                      & 75.92                      & -26.27                                    & -16.00                                    & -18.80                                    & -14.46                                    \\ \cline{2-8} 
                             & vgg19     & 53.22                      & 76.25                      & -26.45                                    & -16.09                                    & -19.14                                    & -14.62                                    \\ \cline{2-8} 
                             & resnet34  & 54.80                      & 77.25                      & -25.25                                    & -15.49                                    & -18.51                                    & -14.16                                    \\ \cline{2-8} 
                             & resnet50  & 61.24                      & 82.62                      & -19.56                                    & -11.03                                    & -14.89                                    & -10.25                                    \\ \cline{2-8} 
                             & resnet101 & 63.05                      & 84.11                      & -18.51                                    & -10.09                                    & -14.32                                    & -9.44                                     \\ \cline{2-8} 
                             & resnet152 & 65.68                      & 86.27                      & -16.12                                    & -8.27                                     & -12.63                                    & -7.78                                     \\ \hline
\multirow{10}{*}{rotate -90} & alexnet   & 27.37                      & 48.87                      & -51.56                                    & -38.19                                    & -29.14                                    & -30.20                                    \\ \cline{2-8} 
                             & vgg11     & 39.98                      & 64.03                      & -42.07                                    & -27.76                                    & -29.04                                    & -24.60                                    \\ \cline{2-8} 
                             & resnet18  & 40.25                      & 64.03                      & -42.29                                    & -28.11                                    & -29.50                                    & -25.04                                    \\ \cline{2-8} 
                             & vgg13     & 41.63                      & 65.58                      & -40.45                                    & -26.52                                    & -28.28                                    & -23.67                                    \\ \cline{2-8} 
                             & vgg16     & 43.04                      & 67.07                      & -39.87                                    & -25.80                                    & -28.54                                    & -23.32                                    \\ \cline{2-8} 
                             & vgg19     & 42.94                      & 67.16                      & -40.66                                    & -26.09                                    & -29.42                                    & -23.71                                    \\ \cline{2-8} 
                             & resnet34  & 44.10                      & 67.61                      & -39.84                                    & -26.04                                    & -29.20                                    & -23.80                                    \\ \cline{2-8} 
                             & resnet50  & 50.14                      & 73.24                      & -34.14                                    & -21.13                                    & -25.99                                    & -19.62                                    \\ \cline{2-8} 
                             & resnet101 & 51.75                      & 74.49                      & -33.11                                    & -20.37                                    & -25.62                                    & -19.05                                    \\ \cline{2-8} 
                             & resnet152 & 53.44                      & 76.21                      & -31.76                                    & -18.97                                    & -24.87                                    & -17.84                                    \\ \hline
\end{tabular}
\label{tab:rotate_neg}
\caption{Drop in accuracy on ImageNet val set by rotating the images (degrees in counter-clockwise direction)}
\end{table*}

==> tables_transformations/scale_in_flip.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{scale by 1.1x} & alexnet   & 55.94                      & 78.69                      & -1.01                                     & -0.48                                     & -0.57                                     & -0.38                                     \\ \cline{2-8} 
                                & vgg11     & 68.10                      & 88.09                      & -1.32                                     & -0.61                                     & -0.91                                     & -0.54                                     \\ \cline{2-8} 
                                & resnet18  & 69.27                      & 88.67                      & -0.69                                     & -0.46                                     & -0.48                                     & -0.41                                     \\ \cline{2-8} 
                                & vgg13     & 69.13                      & 88.78                      & -1.13                                     & -0.52                                     & -0.79                                     & -0.46                                     \\ \cline{2-8} 
                                & vgg16     & 70.99                      & 89.87                      & -0.84                                     & -0.56                                     & -0.60                                     & -0.51                                     \\ \cline{2-8} 
                                & vgg19     & 71.66                      & 90.29                      & -0.98                                     & -0.64                                     & -0.71                                     & -0.59                                     \\ \cline{2-8} 
                                & resnet34  & 72.68                      & 90.89                      & -0.86                                     & -0.58                                     & -0.63                                     & -0.53                                     \\ \cline{2-8} 
                                & resnet50  & 75.38                      & 92.38                      & -0.99                                     & -0.51                                     & -0.75                                     & -0.48                                     \\ \cline{2-8} 
                                & resnet101 & 76.67                      & 93.24                      & -0.91                                     & -0.33                                     & -0.70                                     & -0.31                                     \\ \cline{2-8} 
                                & resnet152 & 77.65                      & 93.66                      & -0.84                                     & -0.41                                     & -0.66                                     & -0.39                                     \\ \hline
\multirow{10}{*}{scale by 1.2x} & alexnet   & 55.09                      & 77.86                      & -2.51                                     & -1.53                                     & -1.42                                     & -1.21                                     \\ \cline{2-8} 
                                & vgg11     & 67.42                      & 87.45                      & -2.31                                     & -1.32                                     & -1.60                                     & -1.17                                     \\ \cline{2-8} 
                                & resnet18  & 68.35                      & 88.14                      & -2.01                                     & -1.05                                     & -1.40                                     & -0.94                                     \\ \cline{2-8} 
                                & vgg13     & 68.33                      & 88.18                      & -2.27                                     & -1.20                                     & -1.59                                     & -1.07                                     \\ \cline{2-8} 
                                & vgg16     & 69.99                      & 89.36                      & -2.24                                     & -1.13                                     & -1.60                                     & -1.02                                     \\ \cline{2-8} 
                                & vgg19     & 70.71                      & 89.61                      & -2.28                                     & -1.39                                     & -1.65                                     & -1.26                                     \\ \cline{2-8} 
                                & resnet34  & 71.83                      & 90.39                      & -2.02                                     & -1.12                                     & -1.48                                     & -1.03                                     \\ \cline{2-8} 
                                & resnet50  & 74.60                      & 91.94                      & -2.00                                     & -0.99                                     & -1.52                                     & -0.92                                     \\ \cline{2-8} 
                                & resnet101 & 75.92                      & 92.78                      & -1.88                                     & -0.82                                     & -1.46                                     & -0.77                                     \\ \cline{2-8} 
                                & resnet152 & 76.97                      & 93.26                      & -1.71                                     & -0.84                                     & -1.34                                     & -0.79                                     \\ \hline
\multirow{10}{*}{scale by 1.3x} & alexnet   & 53.86                      & 76.91                      & -4.69                                     & -2.73                                     & -2.65                                     & -2.16                                     \\ \cline{2-8} 
                                & vgg11     & 66.27                      & 86.77                      & -3.98                                     & -2.09                                     & -2.75                                     & -1.86                                     \\ \cline{2-8} 
                                & resnet18  & 67.38                      & 87.20                      & -3.39                                     & -2.10                                     & -2.37                                     & -1.87                                     \\ \cline{2-8} 
                                & vgg13     & 67.29                      & 87.44                      & -3.76                                     & -2.03                                     & -2.63                                     & -1.81                                     \\ \cline{2-8} 
                                & vgg16     & 68.87                      & 88.35                      & -3.80                                     & -2.25                                     & -2.72                                     & -2.03                                     \\ \cline{2-8} 
                                & vgg19     & 69.79                      & 88.87                      & -3.56                                     & -2.21                                     & -2.58                                     & -2.00                                     \\ \cline{2-8} 
                                & resnet34  & 70.97                      & 89.72                      & -3.19                                     & -1.86                                     & -2.34                                     & -1.70                                     \\ \cline{2-8} 
                                & resnet50  & 73.71                      & 91.22                      & -3.17                                     & -1.77                                     & -2.42                                     & -1.64                                     \\ \cline{2-8} 
                                & resnet101 & 75.04                      & 92.14                      & -3.02                                     & -1.50                                     & -2.33                                     & -1.41                                     \\ \cline{2-8} 
                                & resnet152 & 76.05                      & 92.76                      & -2.89                                     & -1.37                                     & -2.26                                     & -1.29                                     \\ \hline
\multirow{10}{*}{scale by 1.4x} & alexnet   & 52.88                      & 75.89                      & -6.41                                     & -4.02                                     & -3.62                                     & -3.18                                     \\ \cline{2-8} 
                                & vgg11     & 65.03                      & 85.80                      & -5.78                                     & -3.18                                     & -3.99                                     & -2.82                                     \\ \cline{2-8} 
                                & resnet18  & 66.31                      & 86.39                      & -4.93                                     & -3.02                                     & -3.44                                     & -2.69                                     \\ \cline{2-8} 
                                & vgg13     & 65.96                      & 86.31                      & -5.66                                     & -3.29                                     & -3.95                                     & -2.94                                     \\ \cline{2-8} 
                                & vgg16     & 67.81                      & 87.52                      & -5.27                                     & -3.16                                     & -3.78                                     & -2.86                                     \\ \cline{2-8} 
                                & vgg19     & 68.41                      & 88.03                      & -5.47                                     & -3.13                                     & -3.96                                     & -2.85                                     \\ \cline{2-8} 
                                & resnet34  & 69.84                      & 88.85                      & -4.74                                     & -2.81                                     & -3.47                                     & -2.57                                     \\ \cline{2-8} 
                                & resnet50  & 72.66                      & 90.40                      & -4.55                                     & -2.65                                     & -3.47                                     & -2.46                                     \\ \cline{2-8} 
                                & resnet101 & 74.08                      & 91.43                      & -4.25                                     & -2.26                                     & -3.29                                     & -2.12                                     \\ \cline{2-8} 
                                & resnet152 & 75.00                      & 92.08                      & -4.23                                     & -2.09                                     & -3.31                                     & -1.97                                     \\ \hline
\end{tabular}
\label{tab:scale_in1}
\caption{Drop in accuracy on ImageNet val set by scaling in the image by x times.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{scale by 1.6x}   & alexnet   & 50.09                      & 73.47                      & -11.35                                    & -7.08                                     & -6.41                                     & -5.60                                     \\ \cline{2-8} 
                                  & vgg11     & 62.18                      & 83.57                      & -9.90                                     & -5.70                                     & -6.83                                     & -5.05                                     \\ \cline{2-8} 
                                  & resnet18  & 63.68                      & 84.46                      & -8.71                                     & -5.18                                     & -6.08                                     & -4.62                                     \\ \cline{2-8} 
                                  & vgg13     & 63.05                      & 84.24                      & -9.83                                     & -5.60                                     & -6.87                                     & -5.00                                     \\ \cline{2-8} 
                                  & vgg16     & 64.83                      & 85.38                      & -9.44                                     & -5.54                                     & -6.76                                     & -5.00                                     \\ \cline{2-8} 
                                  & vgg19     & 65.67                      & 86.00                      & -9.26                                     & -5.36                                     & -6.70                                     & -4.87                                     \\ \cline{2-8} 
                                  & resnet34  & 67.41                      & 87.10                      & -8.05                                     & -4.72                                     & -5.90                                     & -4.31                                     \\ \cline{2-8} 
                                  & resnet50  & 70.04                      & 88.83                      & -8.00                                     & -4.34                                     & -6.09                                     & -4.03                                     \\ \cline{2-8} 
                                  & resnet101 & 71.75                      & 89.88                      & -7.27                                     & -3.92                                     & -5.63                                     & -3.67                                     \\ \cline{2-8} 
                                  & resnet152 & 72.86                      & 90.60                      & -6.96                                     & -3.67                                     & -5.45                                     & -3.45                                     \\ \hline
\multirow{10}{*}{scale by 1.75x}  & alexnet   & 47.89                      & 71.38                      & -15.25                                    & -9.72                                     & -8.62                                     & -7.68                                     \\ \cline{2-8} 
                                  & vgg11     & 59.95                      & 81.86                      & -13.13                                    & -7.63                                     & -9.06                                     & -6.76                                     \\ \cline{2-8} 
                                  & resnet18  & 61.28                      & 82.76                      & -12.14                                    & -7.08                                     & -8.47                                     & -6.31                                     \\ \cline{2-8} 
                                  & vgg13     & 60.67                      & 82.38                      & -13.23                                    & -7.69                                     & -9.25                                     & -6.86                                     \\ \cline{2-8} 
                                  & vgg16     & 62.65                      & 83.78                      & -12.49                                    & -7.30                                     & -8.94                                     & -6.60                                     \\ \cline{2-8} 
                                  & vgg19     & 63.26                      & 84.19                      & -12.58                                    & -7.36                                     & -9.10                                     & -6.69                                     \\ \cline{2-8} 
                                  & resnet34  & 65.30                      & 85.59                      & -10.92                                    & -6.38                                     & -8.01                                     & -5.83                                     \\ \cline{2-8} 
                                  & resnet50  & 68.09                      & 87.57                      & -10.55                                    & -5.70                                     & -8.03                                     & -5.29                                     \\ \cline{2-8} 
                                  & resnet101 & 70.08                      & 88.56                      & -9.42                                     & -5.33                                     & -7.29                                     & -4.99                                     \\ \cline{2-8} 
                                  & resnet152 & 71.25                      & 89.41                      & -9.01                                     & -4.93                                     & -7.06                                     & -4.63                                     \\ \hline
\multirow{10}{*}{flip left-right} & alexnet   & 56.53                      & 79.18                      & 0.04                                      & 0.15                                      & 0.02                                      & 0.12                                      \\ \cline{2-8} 
                                  & vgg11     & 68.73                      & 88.64                      & -0.41                                     & 0.02                                      & -0.28                                     & 0.01                                      \\ \cline{2-8} 
                                  & resnet18  & 69.53                      & 89.07                      & -0.32                                     & 0.00                                      & -0.22                                     & 0.00                                      \\ \cline{2-8} 
                                  & vgg13     & 69.91                      & 89.27                      & -0.02                                     & 0.03                                      & -0.01                                     & 0.03                                      \\ \cline{2-8} 
                                  & vgg16     & 71.77                      & 90.43                      & 0.26                                      & 0.05                                      & 0.18                                      & 0.04                                      \\ \cline{2-8} 
                                  & vgg19     & 72.45                      & 90.93                      & 0.12                                      & 0.07                                      & 0.09                                      & 0.06                                      \\ \cline{2-8} 
                                  & resnet34  & 73.36                      & 91.44                      & 0.07                                      & 0.02                                      & 0.05                                      & 0.02                                      \\ \cline{2-8} 
                                  & resnet50  & 75.91                      & 92.87                      & -0.29                                     & 0.01                                      & -0.22                                     & 0.01                                      \\ \cline{2-8} 
                                  & resnet101 & 77.21                      & 93.67                      & -0.21                                     & 0.13                                      & -0.16                                     & 0.12                                      \\ \cline{2-8} 
                                  & resnet152 & 78.25                      & 94.03                      & -0.07                                     & -0.02                                     & -0.05                                     & -0.02                                     \\ \hline
\multirow{10}{*}{flip up-down}    & alexnet   & 30.13                      & 53.85                      & -46.69                                    & -31.89                                    & -26.38                                    & -25.22                                    \\ \cline{2-8} 
                                  & vgg11     & 42.87                      & 68.42                      & -37.88                                    & -22.80                                    & -26.14                                    & -20.21                                    \\ \cline{2-8} 
                                  & resnet18  & 41.65                      & 66.85                      & -40.29                                    & -24.95                                    & -28.10                                    & -22.22                                    \\ \cline{2-8} 
                                  & vgg13     & 43.97                      & 69.29                      & -37.12                                    & -22.36                                    & -25.95                                    & -19.95                                    \\ \cline{2-8} 
                                  & vgg16     & 44.50                      & 70.25                      & -37.84                                    & -22.28                                    & -27.09                                    & -20.13                                    \\ \cline{2-8} 
                                  & vgg19     & 44.36                      & 69.99                      & -38.69                                    & -22.98                                    & -28.00                                    & -20.88                                    \\ \cline{2-8} 
                                  & resnet34  & 44.23                      & 69.31                      & -39.66                                    & -24.19                                    & -29.08                                    & -22.11                                    \\ \cline{2-8} 
                                  & resnet50  & 51.57                      & 75.89                      & -32.26                                    & -18.28                                    & -24.56                                    & -16.98                                    \\ \cline{2-8} 
                                  & resnet101 & 53.19                      & 77.23                      & -31.26                                    & -17.44                                    & -24.18                                    & -16.32                                    \\ \cline{2-8} 
                                  & resnet152 & 54.09                      & 78.06                      & -30.93                                    & -17.00                                    & -24.22                                    & -15.99                                    \\ \hline
\end{tabular}
\label{tab:scale_in2_flip}
\caption{Drop in accuracy on ImageNet val set by scaling out the image by x times and flipping the image left-right and up-down.}
\end{table*}

==> tables_transformations/scale_out.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{scale by 0.2x} & alexnet   & 0.63                       & 2.06                       & -98.88                                    & -97.39                                    & -55.87                                    & -77.01                                    \\ \cline{2-8} 
                                & vgg11     & 3.15                       & 8.12                       & -95.44                                    & -90.84                                    & -65.86                                    & -80.51                                    \\ \cline{2-8} 
                                & resnet18  & 2.00                       & 5.85                       & -97.13                                    & -93.43                                    & -67.75                                    & -83.22                                    \\ \cline{2-8} 
                                & vgg13     & 3.68                       & 9.82                       & -94.74                                    & -88.99                                    & -66.24                                    & -79.42                                    \\ \cline{2-8} 
                                & vgg16     & 4.16                       & 10.53                      & -94.19                                    & -88.35                                    & -67.43                                    & -79.85                                    \\ \cline{2-8} 
                                & vgg19     & 3.16                       & 8.19                       & -95.63                                    & -90.99                                    & -69.20                                    & -82.69                                    \\ \cline{2-8} 
                                & resnet34  & 2.56                       & 7.01                       & -96.51                                    & -92.33                                    & -70.75                                    & -84.40                                    \\ \cline{2-8} 
                                & resnet50  & 4.74                       & 11.05                      & -93.77                                    & -88.10                                    & -71.38                                    & -81.81                                    \\ \cline{2-8} 
                                & resnet101 & 6.61                       & 15.56                      & -91.45                                    & -83.37                                    & -70.76                                    & -77.99                                    \\ \cline{2-8} 
                                & resnet152 & 7.53                       & 17.13                      & -90.38                                    & -81.78                                    & -70.78                                    & -76.91                                    \\ \hline
\multirow{10}{*}{scale by 0.3x} & alexnet   & 2.61                       & 6.85                       & -95.38                                    & -91.34                                    & -53.89                                    & -72.22                                    \\ \cline{2-8} 
                                & vgg11     & 15.73                      & 32.06                      & -77.21                                    & -63.82                                    & -53.29                                    & -56.56                                    \\ \cline{2-8} 
                                & resnet18  & 11.25                      & 24.39                      & -83.87                                    & -72.62                                    & -58.50                                    & -64.68                                    \\ \cline{2-8} 
                                & vgg13     & 18.29                      & 36.34                      & -73.84                                    & -59.28                                    & -51.62                                    & -52.90                                    \\ \cline{2-8} 
                                & vgg16     & 20.72                      & 39.58                      & -71.06                                    & -56.21                                    & -50.87                                    & -50.81                                    \\ \cline{2-8} 
                                & vgg19     & 20.25                      & 38.64                      & -72.02                                    & -57.48                                    & -52.12                                    & -52.24                                    \\ \cline{2-8} 
                                & resnet34  & 16.45                      & 32.57                      & -77.55                                    & -64.37                                    & -56.85                                    & -58.84                                    \\ \cline{2-8} 
                                & resnet50  & 25.06                      & 45.19                      & -67.08                                    & -51.33                                    & -51.06                                    & -47.67                                    \\ \cline{2-8} 
                                & resnet101 & 29.62                      & 51.33                      & -61.71                                    & -45.13                                    & -47.75                                    & -42.22                                    \\ \cline{2-8} 
                                & resnet152 & 31.31                      & 53.75                      & -60.02                                    & -42.84                                    & -47.00                                    & -40.29                                    \\ \hline
\multirow{10}{*}{scale by 0.4x} & alexnet   & 8.14                       & 18.31                      & -85.59                                    & -76.84                                    & -48.36                                    & -60.76                                    \\ \cline{2-8} 
                                & vgg11     & 32.00                      & 55.33                      & -53.64                                    & -37.57                                    & -37.02                                    & -33.30                                    \\ \cline{2-8} 
                                & resnet18  & 28.59                      & 50.35                      & -59.01                                    & -43.47                                    & -41.16                                    & -38.72                                    \\ \cline{2-8} 
                                & vgg13     & 36.36                      & 60.40                      & -48.00                                    & -32.32                                    & -33.56                                    & -28.85                                    \\ \cline{2-8} 
                                & vgg16     & 39.86                      & 64.10                      & -44.32                                    & -29.08                                    & -31.73                                    & -26.28                                    \\ \cline{2-8} 
                                & vgg19     & 39.91                      & 64.04                      & -44.85                                    & -29.53                                    & -32.46                                    & -26.83                                    \\ \cline{2-8} 
                                & resnet34  & 36.19                      & 59.70                      & -50.64                                    & -34.70                                    & -37.12                                    & -31.72                                    \\ \cline{2-8} 
                                & resnet50  & 45.67                      & 69.58                      & -40.01                                    & -25.07                                    & -30.46                                    & -23.28                                    \\ \cline{2-8} 
                                & resnet101 & 50.48                      & 74.06                      & -34.75                                    & -20.83                                    & -26.89                                    & -19.48                                    \\ \cline{2-8} 
                                & resnet152 & 52.40                      & 75.95                      & -33.08                                    & -19.25                                    & -25.91                                    & -18.10                                    \\ \hline
\multirow{10}{*}{scale by 0.5x} & alexnet   & 18.40                      & 36.02                      & -67.44                                    & -54.44                                    & -38.11                                    & -43.04                                    \\ \cline{2-8} 
                                & vgg11     & 46.66                      & 71.53                      & -32.39                                    & -19.29                                    & -22.36                                    & -17.10                                    \\ \cline{2-8} 
                                & resnet18  & 45.37                      & 69.92                      & -34.95                                    & -21.51                                    & -24.38                                    & -19.16                                    \\ \cline{2-8} 
                                & vgg13     & 50.00                      & 74.68                      & -28.48                                    & -16.32                                    & -19.92                                    & -14.56                                    \\ \cline{2-8} 
                                & vgg16     & 53.44                      & 77.56                      & -25.35                                    & -14.19                                    & -18.14                                    & -12.82                                    \\ \cline{2-8} 
                                & vgg19     & 53.93                      & 77.65                      & -25.47                                    & -14.55                                    & -18.43                                    & -13.22                                    \\ \cline{2-8} 
                                & resnet34  & 52.42                      & 76.25                      & -28.50                                    & -16.59                                    & -20.89                                    & -15.17                                    \\ \cline{2-8} 
                                & resnet50  & 59.50                      & 82.11                      & -21.84                                    & -11.58                                    & -16.63                                    & -10.75                                    \\ \cline{2-8} 
                                & resnet101 & 62.74                      & 84.48                      & -18.92                                    & -9.69                                     & -14.64                                    & -9.06                                     \\ \cline{2-8} 
                                & resnet152 & 64.45                      & 85.67                      & -17.69                                    & -8.90                                     & -13.85                                    & -8.37                                     \\ \hline
\end{tabular}
\label{tab:scale_out1}
\caption{Drop in accuracy on ImageNet val set by scaling out the image by x times.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{scale by 0.6x} & alexnet   & 32.57                      & 55.63                      & -42.36                                    & -29.64                                    & -23.93                                    & -23.44                                    \\ \cline{2-8} 
                                & vgg11     & 56.46                      & 80.06                      & -18.19                                    & -9.67                                     & -12.55                                    & -8.57                                     \\ \cline{2-8} 
                                & resnet18  & 56.65                      & 79.78                      & -18.78                                    & -10.43                                    & -13.10                                    & -9.29                                     \\ \cline{2-8} 
                                & vgg13     & 59.05                      & 81.88                      & -15.55                                    & -8.25                                     & -10.87                                    & -7.37                                     \\ \cline{2-8} 
                                & vgg16     & 61.69                      & 84.20                      & -13.83                                    & -6.84                                     & -9.90                                     & -6.19                                     \\ \cline{2-8} 
                                & vgg19     & 62.72                      & 84.70                      & -13.33                                    & -6.79                                     & -9.65                                     & -6.17                                     \\ \cline{2-8} 
                                & resnet34  & 62.25                      & 84.16                      & -15.08                                    & -7.94                                     & -11.06                                    & -7.26                                     \\ \cline{2-8} 
                                & resnet50  & 67.48                      & 87.65                      & -11.35                                    & -5.61                                     & -8.64                                     & -5.21                                     \\ \cline{2-8} 
                                & resnet101 & 69.70                      & 89.12                      & -9.92                                     & -4.73                                     & -7.67                                     & -4.42                                     \\ \cline{2-8} 
                                & resnet152 & 71.35                      & 90.18                      & -8.88                                     & -4.11                                     & -6.96                                     & -3.87                                     \\ \hline
\multirow{10}{*}{scale by 0.7x} & alexnet   & 45.34                      & 69.41                      & -19.76                                    & -12.22                                    & -11.17                                    & -9.66                                     \\ \cline{2-8} 
                                & vgg11     & 63.57                      & 85.35                      & -7.89                                     & -3.69                                     & -5.45                                     & -3.27                                     \\ \cline{2-8} 
                                & resnet18  & 63.66                      & 85.02                      & -8.73                                     & -4.56                                     & -6.09                                     & -4.06                                     \\ \cline{2-8} 
                                & vgg13     & 65.30                      & 86.53                      & -6.60                                     & -3.05                                     & -4.61                                     & -2.72                                     \\ \cline{2-8} 
                                & vgg16     & 67.26                      & 87.77                      & -6.05                                     & -2.89                                     & -4.33                                     & -2.61                                     \\ \cline{2-8} 
                                & vgg19     & 68.02                      & 88.32                      & -6.01                                     & -2.81                                     & -4.35                                     & -2.55                                     \\ \cline{2-8} 
                                & resnet34  & 68.07                      & 88.20                      & -7.14                                     & -3.52                                     & -5.24                                     & -3.22                                     \\ \cline{2-8} 
                                & resnet50  & 72.11                      & 90.56                      & -5.28                                     & -2.47                                     & -4.02                                     & -2.30                                     \\ \cline{2-8} 
                                & resnet101 & 73.79                      & 91.67                      & -4.63                                     & -2.00                                     & -3.59                                     & -1.87                                     \\ \cline{2-8} 
                                & resnet152 & 75.14                      & 92.59                      & -4.04                                     & -1.54                                     & -3.17                                     & -1.45                                     \\ \hline
\multirow{10}{*}{scale by 0.8x} & alexnet   & 51.72                      & 75.28                      & -8.47                                     & -4.79                                     & -4.78                                     & -3.79                                     \\ \cline{2-8} 
                                & vgg11     & 66.52                      & 87.38                      & -3.61                                     & -1.41                                     & -2.49                                     & -1.25                                     \\ \cline{2-8} 
                                & resnet18  & 66.96                      & 87.33                      & -4.01                                     & -1.96                                     & -2.80                                     & -1.74                                     \\ \cline{2-8} 
                                & vgg13     & 67.92                      & 88.04                      & -2.85                                     & -1.35                                     & -2.00                                     & -1.21                                     \\ \cline{2-8} 
                                & vgg16     & 69.50                      & 89.25                      & -2.92                                     & -1.25                                     & -2.09                                     & -1.13                                     \\ \cline{2-8} 
                                & vgg19     & 70.37                      & 89.69                      & -2.75                                     & -1.30                                     & -1.99                                     & -1.18                                     \\ \cline{2-8} 
                                & resnet34  & 70.78                      & 89.86                      & -3.45                                     & -1.71                                     & -2.53                                     & -1.56                                     \\ \cline{2-8} 
                                & resnet50  & 74.23                      & 91.97                      & -2.49                                     & -0.96                                     & -1.89                                     & -0.89                                     \\ \cline{2-8} 
                                & resnet101 & 75.75                      & 92.81                      & -2.09                                     & -0.79                                     & -1.62                                     & -0.74                                     \\ \cline{2-8} 
                                & resnet152 & 76.88                      & 93.53                      & -1.82                                     & -0.55                                     & -1.43                                     & -0.52                                     \\ \hline
\multirow{10}{*}{scale by 0.9x} & alexnet   & 55.59                      & 78.43                      & -1.63                                     & -0.81                                     & -0.92                                     & -0.64                                     \\ \cline{2-8} 
                                & vgg11     & 68.52                      & 88.52                      & -0.72                                     & -0.12                                     & -0.49                                     & -0.10                                     \\ \cline{2-8} 
                                & resnet18  & 69.26                      & 88.85                      & -0.71                                     & -0.25                                     & -0.49                                     & -0.22                                     \\ \cline{2-8} 
                                & vgg13     & 69.50                      & 89.07                      & -0.60                                     & -0.19                                     & -0.42                                     & -0.17                                     \\ \cline{2-8} 
                                & vgg16     & 71.50                      & 90.31                      & -0.13                                     & -0.08                                     & -0.09                                     & -0.07                                     \\ \cline{2-8} 
                                & vgg19     & 72.09                      & 90.71                      & -0.39                                     & -0.18                                     & -0.28                                     & -0.16                                     \\ \cline{2-8} 
                                & resnet34  & 72.75                      & 91.00                      & -0.76                                     & -0.46                                     & -0.56                                     & -0.42                                     \\ \cline{2-8} 
                                & resnet50  & 75.52                      & 92.67                      & -0.80                                     & -0.20                                     & -0.61                                     & -0.19                                     \\ \cline{2-8} 
                                & resnet101 & 76.99                      & 93.42                      & -0.49                                     & -0.13                                     & -0.38                                     & -0.12                                     \\ \cline{2-8} 
                                & resnet152 & 78.00                      & 93.97                      & -0.40                                     & -0.08                                     & -0.31                                     & -0.07                                     \\ \hline
\end{tabular}
\label{tab:scale_out2}
\caption{Drop in accuracy on ImageNet val set by scaling out the image by x times.}
\end{table*}

==> tables_transformations/translate_x.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{translate in x by 2\%}  & alexnet   & 56.38                      & 79.08                      & -0.23                                     & 0.02                                      & -0.13                                     & 0.01                                      \\ \cline{2-8} 
                                         & vgg11     & 68.88                      & 88.62                      & -0.19                                     & 0.00                                      & -0.13                                     & 0.00                                      \\ \cline{2-8} 
                                         & resnet18  & 69.59                      & 89.01                      & -0.24                                     & -0.07                                     & -0.16                                     & -0.06                                     \\ \cline{2-8} 
                                         & vgg13     & 69.72                      & 89.25                      & -0.28                                     & 0.00                                      & -0.20                                     & 0.00                                      \\ \cline{2-8} 
                                         & vgg16     & 71.59                      & 90.38                      & 0.01                                      & 0.00                                      & 0.01                                      & 0.00                                      \\ \cline{2-8} 
                                         & vgg19     & 72.30                      & 90.79                      & -0.09                                     & -0.09                                     & -0.06                                     & -0.09                                     \\ \cline{2-8} 
                                         & resnet34  & 73.25                      & 91.27                      & -0.08                                     & -0.16                                     & -0.06                                     & -0.15                                     \\ \cline{2-8} 
                                         & resnet50  & 75.90                      & 92.82                      & -0.29                                     & -0.04                                     & -0.22                                     & -0.04                                     \\ \cline{2-8} 
                                         & resnet101 & 77.22                      & 93.45                      & -0.19                                     & -0.10                                     & -0.15                                     & -0.09                                     \\ \cline{2-8} 
                                         & resnet152 & 78.24                      & 94.05                      & -0.08                                     & 0.00                                      & -0.07                                     & 0.00                                      \\ \hline
\multirow{10}{*}{translate in x by 5\%}  & alexnet   & 56.27                      & 78.93                      & -0.41                                     & -0.18                                     & -0.23                                     & -0.14                                     \\ \cline{2-8} 
                                         & vgg11     & 68.75                      & 88.58                      & -0.38                                     & -0.05                                     & -0.26                                     & -0.05                                     \\ \cline{2-8} 
                                         & resnet18  & 69.54                      & 88.89                      & -0.31                                     & -0.20                                     & -0.22                                     & -0.18                                     \\ \cline{2-8} 
                                         & vgg13     & 69.75                      & 89.25                      & -0.25                                     & 0.00                                      & -0.17                                     & 0.00                                      \\ \cline{2-8} 
                                         & vgg16     & 71.48                      & 90.34                      & -0.15                                     & -0.05                                     & -0.10                                     & -0.04                                     \\ \cline{2-8} 
                                         & vgg19     & 72.15                      & 90.74                      & -0.29                                     & -0.15                                     & -0.21                                     & -0.14                                     \\ \cline{2-8} 
                                         & resnet34  & 73.03                      & 91.15                      & -0.38                                     & -0.29                                     & -0.28                                     & -0.26                                     \\ \cline{2-8} 
                                         & resnet50  & 75.80                      & 92.70                      & -0.43                                     & -0.17                                     & -0.33                                     & -0.16                                     \\ \cline{2-8} 
                                         & resnet101 & 77.09                      & 93.51                      & -0.37                                     & -0.04                                     & -0.29                                     & -0.04                                     \\ \cline{2-8} 
                                         & resnet152 & 78.12                      & 94.00                      & -0.24                                     & -0.05                                     & -0.19                                     & -0.05                                     \\ \hline
\multirow{10}{*}{translate in x by 10\%} & alexnet   & 55.25                      & 78.21                      & -2.22                                     & -1.08                                     & -1.25                                     & -0.86                                     \\ \cline{2-8} 
                                         & vgg11     & 68.12                      & 88.19                      & -1.30                                     & -0.49                                     & -0.90                                     & -0.43                                     \\ \cline{2-8} 
                                         & resnet18  & 68.94                      & 88.40                      & -1.16                                     & -0.75                                     & -0.81                                     & -0.67                                     \\ \cline{2-8} 
                                         & vgg13     & 69.13                      & 88.68                      & -1.13                                     & -0.63                                     & -0.79                                     & -0.56                                     \\ \cline{2-8} 
                                         & vgg16     & 70.85                      & 89.92                      & -1.04                                     & -0.51                                     & -0.74                                     & -0.46                                     \\ \cline{2-8} 
                                         & vgg19     & 71.66                      & 90.40                      & -0.98                                     & -0.52                                     & -0.71                                     & -0.47                                     \\ \cline{2-8} 
                                         & resnet34  & 72.56                      & 90.85                      & -1.01                                     & -0.62                                     & -0.74                                     & -0.57                                     \\ \cline{2-8} 
                                         & resnet50  & 75.41                      & 92.39                      & -0.94                                     & -0.51                                     & -0.71                                     & -0.47                                     \\ \cline{2-8} 
                                         & resnet101 & 76.79                      & 93.16                      & -0.75                                     & -0.41                                     & -0.58                                     & -0.39                                     \\ \cline{2-8} 
                                         & resnet152 & 77.79                      & 93.72                      & -0.66                                     & -0.35                                     & -0.52                                     & -0.33                                     \\ \hline
\multirow{10}{*}{translate in x by 15\%} & alexnet   & 53.73                      & 76.86                      & -4.91                                     & -2.79                                     & -2.77                                     & -2.20                                     \\ \cline{2-8} 
                                         & vgg11     & 67.18                      & 87.45                      & -2.65                                     & -1.32                                     & -1.83                                     & -1.17                                     \\ \cline{2-8} 
                                         & resnet18  & 67.96                      & 87.81                      & -2.57                                     & -1.42                                     & -1.80                                     & -1.26                                     \\ \cline{2-8} 
                                         & vgg13     & 68.19                      & 88.10                      & -2.47                                     & -1.28                                     & -1.73                                     & -1.14                                     \\ \cline{2-8} 
                                         & vgg16     & 69.93                      & 89.34                      & -2.32                                     & -1.15                                     & -1.66                                     & -1.04                                     \\ \cline{2-8} 
                                         & vgg19     & 70.54                      & 89.68                      & -2.52                                     & -1.31                                     & -1.82                                     & -1.19                                     \\ \cline{2-8} 
                                         & resnet34  & 71.58                      & 90.23                      & -2.36                                     & -1.30                                     & -1.73                                     & -1.19                                     \\ \cline{2-8} 
                                         & resnet50  & 74.46                      & 91.85                      & -2.19                                     & -1.09                                     & -1.67                                     & -1.01                                     \\ \cline{2-8} 
                                         & resnet101 & 75.87                      & 92.68                      & -1.94                                     & -0.93                                     & -1.50                                     & -0.87                                     \\ \cline{2-8} 
                                         & resnet152 & 77.00                      & 93.27                      & -1.67                                     & -0.82                                     & -1.31                                     & -0.77                                     \\ \hline
\end{tabular}
\label{tab:translate_x1}
\caption{Drop in accuracy on ImageNet val set by translating the image in horizontal direction by x\% of width of the image.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{translate in x by 20\%} & alexnet   & 50.98                      & 74.61                      & -9.79                                     & -5.63                                     & -5.53                                     & -4.45                                     \\ \cline{2-8} 
                                         & vgg11     & 65.33                      & 86.31                      & -5.34                                     & -2.61                                     & -3.68                                     & -2.31                                     \\ \cline{2-8} 
                                         & resnet18  & 66.28                      & 86.61                      & -4.98                                     & -2.76                                     & -3.47                                     & -2.46                                     \\ \cline{2-8} 
                                         & vgg13     & 66.40                      & 86.94                      & -5.03                                     & -2.58                                     & -3.51                                     & -2.30                                     \\ \cline{2-8} 
                                         & vgg16     & 68.16                      & 88.33                      & -4.79                                     & -2.27                                     & -3.43                                     & -2.05                                     \\ \cline{2-8} 
                                         & vgg19     & 69.17                      & 88.72                      & -4.41                                     & -2.37                                     & -3.19                                     & -2.15                                     \\ \cline{2-8} 
                                         & resnet34  & 70.18                      & 89.26                      & -4.27                                     & -2.36                                     & -3.13                                     & -2.16                                     \\ \cline{2-8} 
                                         & resnet50  & 73.01                      & 90.95                      & -4.10                                     & -2.05                                     & -3.12                                     & -1.91                                     \\ \cline{2-8} 
                                         & resnet101 & 74.48                      & 91.76                      & -3.74                                     & -1.90                                     & -2.89                                     & -1.78                                     \\ \cline{2-8} 
                                         & resnet152 & 75.79                      & 92.57                      & -3.22                                     & -1.57                                     & -2.52                                     & -1.48                                     \\ \hline
\multirow{10}{*}{translate in x by 25\%} & alexnet   & 46.99                      & 71.27                      & -16.84                                    & -9.87                                     & -9.52                                     & -7.80                                     \\ \cline{2-8} 
                                         & vgg11     & 62.76                      & 84.52                      & -9.06                                     & -4.63                                     & -6.25                                     & -4.10                                     \\ \cline{2-8} 
                                         & resnet18  & 63.76                      & 84.67                      & -8.60                                     & -4.94                                     & -6.00                                     & -4.40                                     \\ \cline{2-8} 
                                         & vgg13     & 64.19                      & 85.28                      & -8.20                                     & -4.45                                     & -5.73                                     & -3.97                                     \\ \cline{2-8} 
                                         & vgg16     & 66.06                      & 86.73                      & -7.72                                     & -4.04                                     & -5.53                                     & -3.65                                     \\ \cline{2-8} 
                                         & vgg19     & 66.83                      & 87.21                      & -7.65                                     & -4.03                                     & -5.54                                     & -3.66                                     \\ \cline{2-8} 
                                         & resnet34  & 67.95                      & 87.89                      & -7.31                                     & -3.86                                     & -5.36                                     & -3.53                                     \\ \cline{2-8} 
                                         & resnet50  & 71.17                      & 89.59                      & -6.51                                     & -3.53                                     & -4.95                                     & -3.28                                     \\ \cline{2-8} 
                                         & resnet101 & 72.66                      & 90.64                      & -6.09                                     & -3.10                                     & -4.71                                     & -2.90                                     \\ \cline{2-8} 
                                         & resnet152 & 74.00                      & 91.47                      & -5.50                                     & -2.74                                     & -4.31                                     & -2.58                                     \\ \hline
\multirow{10}{*}{translate in x by 35\%} & alexnet   & 36.47                      & 60.45                      & -35.45                                    & -23.55                                    & -20.03                                    & -18.62                                    \\ \cline{2-8} 
                                         & vgg11     & 55.51                      & 78.54                      & -19.56                                    & -11.38                                    & -13.50                                    & -10.09                                    \\ \cline{2-8} 
                                         & resnet18  & 56.56                      & 78.86                      & -18.92                                    & -11.46                                    & -13.20                                    & -10.21                                    \\ \cline{2-8} 
                                         & vgg13     & 57.20                      & 79.86                      & -18.19                                    & -10.51                                    & -12.72                                    & -9.38                                     \\ \cline{2-8} 
                                         & vgg16     & 59.34                      & 81.40                      & -17.11                                    & -9.94                                     & -12.25                                    & -8.99                                     \\ \cline{2-8} 
                                         & vgg19     & 60.05                      & 81.90                      & -17.02                                    & -9.87                                     & -12.31                                    & -8.97                                     \\ \cline{2-8} 
                                         & resnet34  & 61.30                      & 82.81                      & -16.38                                    & -9.42                                     & -12.01                                    & -8.61                                     \\ \cline{2-8} 
                                         & resnet50  & 64.51                      & 84.99                      & -15.26                                    & -8.48                                     & -11.61                                    & -7.87                                     \\ \cline{2-8} 
                                         & resnet101 & 66.49                      & 86.39                      & -14.07                                    & -7.65                                     & -10.89                                    & -7.15                                     \\ \cline{2-8} 
                                         & resnet152 & 67.77                      & 87.10                      & -13.45                                    & -7.39                                     & -10.54                                    & -6.95                                     \\ \hline
\multirow{10}{*}{translate in x by 50\%} & alexnet   & 18.28                      & 36.42                      & -67.64                                    & -53.93                                    & -38.22                                    & -42.64                                    \\ \cline{2-8} 
                                         & vgg11     & 37.61                      & 60.73                      & -45.51                                    & -31.48                                    & -31.40                                    & -27.90                                    \\ \cline{2-8} 
                                         & resnet18  & 37.14                      & 59.64                      & -46.75                                    & -33.04                                    & -32.61                                    & -29.43                                    \\ \cline{2-8} 
                                         & vgg13     & 39.69                      & 62.81                      & -43.24                                    & -29.62                                    & -30.23                                    & -26.44                                    \\ \cline{2-8} 
                                         & vgg16     & 41.54                      & 64.52                      & -41.98                                    & -28.62                                    & -30.05                                    & -25.87                                    \\ \cline{2-8} 
                                         & vgg19     & 42.12                      & 64.97                      & -41.80                                    & -28.51                                    & -30.25                                    & -25.90                                    \\ \cline{2-8} 
                                         & resnet34  & 42.96                      & 65.63                      & -41.40                                    & -28.21                                    & -30.35                                    & -25.79                                    \\ \cline{2-8} 
                                         & resnet50  & 46.83                      & 68.95                      & -38.49                                    & -25.75                                    & -29.30                                    & -23.91                                    \\ \cline{2-8} 
                                         & resnet101 & 48.55                      & 70.85                      & -37.25                                    & -24.27                                    & -28.82                                    & -22.70                                    \\ \cline{2-8} 
                                         & resnet152 & 50.18                      & 72.00                      & -35.92                                    & -23.44                                    & -28.13                                    & -22.04                                    \\ \hline
\end{tabular}
\label{tab:translate_x2}
\caption{Drop in accuracy on ImageNet val set by translating the image in horizontal direction by x\% of width of the image.}
\end{table*}

==> tables_transformations/translate_y.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{translate in y by 2\%}  & alexnet   & 56.26                      & 79.01                      & -0.44                                     & -0.07                                     & -0.25                                     & -0.05                                     \\ \cline{2-8} 
                                         & vgg11     & 68.67                      & 88.51                      & -0.50                                     & -0.13                                     & -0.34                                     & -0.11                                     \\ \cline{2-8} 
                                         & resnet18  & 69.46                      & 89.00                      & -0.42                                     & -0.09                                     & -0.29                                     & -0.08                                     \\ \cline{2-8} 
                                         & vgg13     & 69.70                      & 89.25                      & -0.32                                     & 0.01                                      & -0.22                                     & 0.01                                      \\ \cline{2-8} 
                                         & vgg16     & 71.46                      & 90.35                      & -0.18                                     & -0.04                                     & -0.13                                     & -0.04                                     \\ \cline{2-8} 
                                         & vgg19     & 72.07                      & 90.79                      & -0.41                                     & -0.10                                     & -0.30                                     & -0.09                                     \\ \cline{2-8} 
                                         & resnet34  & 73.12                      & 91.30                      & -0.26                                     & -0.13                                     & -0.19                                     & -0.12                                     \\ \cline{2-8} 
                                         & resnet50  & 75.82                      & 92.77                      & -0.40                                     & -0.10                                     & -0.31                                     & -0.09                                     \\ \cline{2-8} 
                                         & resnet101 & 77.07                      & 93.41                      & -0.39                                     & -0.15                                     & -0.30                                     & -0.14                                     \\ \cline{2-8} 
                                         & resnet152 & 78.17                      & 94.01                      & -0.17                                     & -0.04                                     & -0.13                                     & -0.04                                     \\ \hline
\multirow{10}{*}{translate in y by 5\%}  & alexnet   & 55.97                      & 78.83                      & -0.95                                     & -0.30                                     & -0.53                                     & -0.24                                     \\ \cline{2-8} 
                                         & vgg11     & 68.47                      & 88.46                      & -0.79                                     & -0.19                                     & -0.55                                     & -0.17                                     \\ \cline{2-8} 
                                         & resnet18  & 69.34                      & 88.85                      & -0.59                                     & -0.25                                     & -0.41                                     & -0.23                                     \\ \cline{2-8} 
                                         & vgg13     & 69.58                      & 89.07                      & -0.48                                     & -0.19                                     & -0.33                                     & -0.17                                     \\ \cline{2-8} 
                                         & vgg16     & 71.29                      & 90.32                      & -0.42                                     & -0.07                                     & -0.30                                     & -0.06                                     \\ \cline{2-8} 
                                         & vgg19     & 71.97                      & 90.67                      & -0.55                                     & -0.22                                     & -0.40                                     & -0.20                                     \\ \cline{2-8} 
                                         & resnet34  & 72.88                      & 91.16                      & -0.58                                     & -0.29                                     & -0.43                                     & -0.26                                     \\ \cline{2-8} 
                                         & resnet50  & 75.51                      & 92.73                      & -0.81                                     & -0.14                                     & -0.61                                     & -0.13                                     \\ \cline{2-8} 
                                         & resnet101 & 76.87                      & 93.37                      & -0.65                                     & -0.19                                     & -0.50                                     & -0.18                                     \\ \cline{2-8} 
                                         & resnet152 & 78.12                      & 93.90                      & -0.25                                     & -0.16                                     & -0.19                                     & -0.15                                     \\ \hline
\multirow{10}{*}{translate in y by 10\%} & alexnet   & 53.96                      & 77.41                      & -4.51                                     & -2.09                                     & -2.55                                     & -1.65                                     \\ \cline{2-8} 
                                         & vgg11     & 67.49                      & 87.80                      & -2.21                                     & -0.93                                     & -1.52                                     & -0.82                                     \\ \cline{2-8} 
                                         & resnet18  & 68.17                      & 88.22                      & -2.26                                     & -0.95                                     & -1.58                                     & -0.85                                     \\ \cline{2-8} 
                                         & vgg13     & 68.42                      & 88.39                      & -2.14                                     & -0.96                                     & -1.49                                     & -0.86                                     \\ \cline{2-8} 
                                         & vgg16     & 70.25                      & 89.57                      & -1.87                                     & -0.89                                     & -1.34                                     & -0.81                                     \\ \cline{2-8} 
                                         & vgg19     & 71.07                      & 90.09                      & -1.79                                     & -0.86                                     & -1.30                                     & -0.78                                     \\ \cline{2-8} 
                                         & resnet34  & 72.08                      & 90.51                      & -1.68                                     & -0.99                                     & -1.23                                     & -0.91                                     \\ \cline{2-8} 
                                         & resnet50  & 74.83                      & 92.18                      & -1.71                                     & -0.74                                     & -1.30                                     & -0.69                                     \\ \cline{2-8} 
                                         & resnet101 & 76.33                      & 93.03                      & -1.35                                     & -0.55                                     & -1.05                                     & -0.51                                     \\ \cline{2-8} 
                                         & resnet152 & 77.37                      & 93.60                      & -1.20                                     & -0.48                                     & -0.94                                     & -0.45                                     \\ \hline
\multirow{10}{*}{translate in y by 15\%} & alexnet   & 51.53                      & 75.37                      & -8.81                                     & -4.67                                     & -4.98                                     & -3.70                                     \\ \cline{2-8} 
                                         & vgg11     & 65.93                      & 86.84                      & -4.46                                     & -2.02                                     & -3.08                                     & -1.79                                     \\ \cline{2-8} 
                                         & resnet18  & 67.00                      & 87.38                      & -3.94                                     & -1.91                                     & -2.75                                     & -1.70                                     \\ \cline{2-8} 
                                         & vgg13     & 67.05                      & 87.38                      & -4.11                                     & -2.09                                     & -2.87                                     & -1.87                                     \\ \cline{2-8} 
                                         & vgg16     & 69.11                      & 88.88                      & -3.46                                     & -1.66                                     & -2.47                                     & -1.50                                     \\ \cline{2-8} 
                                         & vgg19     & 69.70                      & 89.28                      & -3.69                                     & -1.75                                     & -2.67                                     & -1.59                                     \\ \cline{2-8} 
                                         & resnet34  & 70.61                      & 89.83                      & -3.68                                     & -1.73                                     & -2.70                                     & -1.59                                     \\ \cline{2-8} 
                                         & resnet50  & 73.94                      & 91.65                      & -2.88                                     & -1.30                                     & -2.19                                     & -1.21                                     \\ \cline{2-8} 
                                         & resnet101 & 75.37                      & 92.27                      & -2.59                                     & -1.36                                     & -2.00                                     & -1.27                                     \\ \cline{2-8} 
                                         & resnet152 & 76.47                      & 92.89                      & -2.35                                     & -1.22                                     & -1.84                                     & -1.15                                     \\ \hline
\end{tabular}
\label{tab:translate_y1}
\caption{Drop in accuracy on ImageNet val set by translating the image in horizontal direction by x\% of height of the image.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{|l|l|r|r|r|r|r|r|}
\hline
\parbox{1.5cm}{Transformation}               & Model      & \multicolumn{1}{l|}{Top 1} & \multicolumn{1}{l|}{Top 5} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Rel. \% change in Top5}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top1}} & \multicolumn{1}{l|}{\parbox{1.5cm}{Abs. \% change in Top5}} \\ \hline
\multirow{10}{*}{translate in y by 20\%} & alexnet   & 48.09                      & 72.27                      & -14.90                                    & -8.60                                     & -8.42                                     & -6.80                                     \\ \cline{2-8} 
                                         & vgg11     & 63.63                      & 85.26                      & -7.80                                     & -3.80                                     & -5.38                                     & -3.37                                     \\ \cline{2-8} 
                                         & resnet18  & 65.37                      & 86.23                      & -6.28                                     & -3.20                                     & -4.38                                     & -2.85                                     \\ \cline{2-8} 
                                         & vgg13     & 65.07                      & 86.20                      & -6.93                                     & -3.41                                     & -4.85                                     & -3.05                                     \\ \cline{2-8} 
                                         & vgg16     & 67.26                      & 87.46                      & -6.05                                     & -3.23                                     & -4.33                                     & -2.92                                     \\ \cline{2-8} 
                                         & vgg19     & 68.09                      & 88.06                      & -5.91                                     & -3.09                                     & -4.28                                     & -2.81                                     \\ \cline{2-8} 
                                         & resnet34  & 69.29                      & 88.67                      & -5.48                                     & -3.01                                     & -4.02                                     & -2.75                                     \\ \cline{2-8} 
                                         & resnet50  & 72.35                      & 90.63                      & -4.96                                     & -2.41                                     & -3.78                                     & -2.23                                     \\ \cline{2-8} 
                                         & resnet101 & 74.04                      & 91.54                      & -4.31                                     & -2.15                                     & -3.33                                     & -2.01                                     \\ \cline{2-8} 
                                         & resnet152 & 75.30                      & 92.19                      & -3.85                                     & -1.97                                     & -3.01                                     & -1.85                                     \\ \hline
\multirow{10}{*}{translate in y by 25\%} & alexnet   & 43.47                      & 67.67                      & -23.06                                    & -14.42                                    & -13.03                                    & -11.40                                    \\ \cline{2-8} 
                                         & vgg11     & 61.06                      & 83.15                      & -11.52                                    & -6.18                                     & -7.95                                     & -5.48                                     \\ \cline{2-8} 
                                         & resnet18  & 62.73                      & 84.16                      & -10.07                                    & -5.52                                     & -7.02                                     & -4.92                                     \\ \cline{2-8} 
                                         & vgg13     & 62.64                      & 84.11                      & -10.41                                    & -5.75                                     & -7.28                                     & -5.13                                     \\ \cline{2-8} 
                                         & vgg16     & 64.81                      & 85.69                      & -9.46                                     & -5.19                                     & -6.77                                     & -4.69                                     \\ \cline{2-8} 
                                         & vgg19     & 65.60                      & 86.38                      & -9.35                                     & -4.95                                     & -6.77                                     & -4.50                                     \\ \cline{2-8} 
                                         & resnet34  & 67.17                      & 87.01                      & -8.37                                     & -4.82                                     & -6.14                                     & -4.41                                     \\ \cline{2-8} 
                                         & resnet50  & 70.37                      & 89.32                      & -7.56                                     & -3.82                                     & -5.75                                     & -3.54                                     \\ \cline{2-8} 
                                         & resnet101 & 72.24                      & 90.19                      & -6.64                                     & -3.59                                     & -5.14                                     & -3.36                                     \\ \cline{2-8} 
                                         & resnet152 & 73.29                      & 90.82                      & -6.41                                     & -3.43                                     & -5.02                                     & -3.23                                     \\ \hline
\multirow{10}{*}{translate in y by 35\%} & alexnet   & 33.75                      & 57.22                      & -40.28                                    & -27.63                                    & -22.76                                    & -21.84                                    \\ \cline{2-8} 
                                         & vgg11     & 53.80                      & 77.13                      & -22.04                                    & -12.98                                    & -15.21                                    & -11.50                                    \\ \cline{2-8} 
                                         & resnet18  & 56.04                      & 78.23                      & -19.66                                    & -12.17                                    & -13.72                                    & -10.84                                    \\ \cline{2-8} 
                                         & vgg13     & 55.51                      & 78.28                      & -20.61                                    & -12.29                                    & -14.41                                    & -10.96                                    \\ \cline{2-8} 
                                         & vgg16     & 57.68                      & 80.09                      & -19.42                                    & -11.38                                    & -13.90                                    & -10.29                                    \\ \cline{2-8} 
                                         & vgg19     & 59.09                      & 80.90                      & -18.34                                    & -10.98                                    & -13.27                                    & -9.98                                     \\ \cline{2-8} 
                                         & resnet34  & 60.57                      & 81.80                      & -17.37                                    & -10.52                                    & -12.74                                    & -9.62                                     \\ \cline{2-8} 
                                         & resnet50  & 64.48                      & 84.50                      & -15.30                                    & -9.01                                     & -11.65                                    & -8.37                                     \\ \cline{2-8} 
                                         & resnet101 & 66.35                      & 85.88                      & -14.25                                    & -8.19                                     & -11.03                                    & -7.66                                     \\ \cline{2-8} 
                                         & resnet152 & 67.66                      & 86.83                      & -13.60                                    & -7.67                                     & -10.65                                    & -7.21                                     \\ \hline
\multirow{10}{*}{translate in y by 50\%} & alexnet   & 17.50                      & 35.47                      & -69.04                                    & -55.13                                    & -39.01                                    & -43.59                                    \\ \cline{2-8} 
                                         & vgg11     & 37.32                      & 60.45                      & -45.92                                    & -31.79                                    & -31.69                                    & -28.18                                    \\ \cline{2-8} 
                                         & resnet18  & 38.07                      & 60.59                      & -45.43                                    & -31.98                                    & -31.69                                    & -28.49                                    \\ \cline{2-8} 
                                         & vgg13     & 39.11                      & 62.33                      & -44.06                                    & -30.16                                    & -30.80                                    & -26.92                                    \\ \cline{2-8} 
                                         & vgg16     & 41.79                      & 64.72                      & -41.62                                    & -28.40                                    & -29.79                                    & -25.67                                    \\ \cline{2-8} 
                                         & vgg19     & 42.45                      & 65.56                      & -41.34                                    & -27.86                                    & -29.91                                    & -25.32                                    \\ \cline{2-8} 
                                         & resnet34  & 43.18                      & 65.91                      & -41.10                                    & -27.91                                    & -30.13                                    & -25.51                                    \\ \cline{2-8} 
                                         & resnet50  & 48.05                      & 70.05                      & -36.88                                    & -24.56                                    & -28.08                                    & -22.81                                    \\ \cline{2-8} 
                                         & resnet101 & 50.16                      & 71.66                      & -35.17                                    & -23.39                                    & -27.21                                    & -21.88                                    \\ \cline{2-8} 
                                         & resnet152 & 51.53                      & 72.86                      & -34.19                                    & -22.53                                    & -26.77                                    & -21.19                                    \\ \hline
\end{tabular}
\label{tab:translate_y2}
\caption{Drop in accuracy on ImageNet val set by translating the image in horizontal direction by x\% of height of the image.}
\end{table*}
